Evaluating financial tail risk forecasts: Testing Equal Predictive Ability

This paper provides comprehensive simulation results on the finite sample properties of the Diebold-Mariano (DM) test by Diebold and Mariano (1995) and the model confidence set (MCS) testing procedure by Hansen et al. (2011) applied to the asymmetric loss functions specific to financial tail risk forecasts, such as Value-at-Risk (VaR) and Expected Shortfall (ES). We focus on statistical loss functions that are strictly consistent in the sense of Gneiting (2011a). We find that the tests show little power against models that underestimate the tail risk at the most extreme quantile levels, while the finite sample properties generally improve with the quantile level and the out-of-sample size. For the small quantile levels and out-of-sample sizes of up to two years, we observe heavily skewed test statistics and non-negligible type III errors, which implies that researchers should be cautious about using standard normal or bootstrapped critical values. We demonstrate both empirically and theoretically how these unfavorable finite sample results relate to the asymmetric loss functions and the time varying volatility inherent in financial return data.

==> content/tables/simulation_true_model_10/summary_statistics/0/0/panel_mcs_75.tex <==
\begin{table}[h!]
\scriptsize
\centering
\caption{Simulation results for the second set of models: VaR evaluated using the GPL loss with \(b=0.5\).}
\label{tab:second}
\begin{tabularx}{1\textwidth}{l X X X X X X X X X }
\toprule 
        &  & \multicolumn{4}{c}{Potency} & \multicolumn{4}{c}{Power}   \\ 
                               &\(p \backslash P \) & 63 & 126 & 251 & 500 & 63 & 126 & 251 & 500   \\ 
\toprule 
\multirow{ 4}{*}{\( \nu=3\)}   &  0.010 &  0.573 &  0.796 &  0.912 &  0.945 &  6.539 &  8.228 &  8.959 &  8.947   \\ 
                               &  0.025 &  0.851 &  0.937 &  0.968 &  0.982 &  7.595 &  8.464 &  8.768 &  8.540   \\ 
                               &  0.050 &  0.908 &  0.968 &  0.984 &  0.992 &  7.674 &  8.262 &  8.255 &  8.078   \\ 
                               &  0.100 &  0.938 &  0.955 &  0.984 &  0.997 &  7.553 &  7.583 &  7.277 &  6.532   \\ 
\bottomrule 
\multirow{ 4}{*}{\( \nu=7\)}   &  0.010 &  0.581 &  0.767 &  0.901 &  0.958 &  6.312 &  7.726 &  8.583 &  8.711   \\ 
                               &  0.025 &  0.782 &  0.890 &  0.949 &  0.978 &  7.706 &  8.514 &  8.836 &  8.431   \\ 
                               &  0.050 &  0.847 &  0.918 &  0.972 &  0.979 &  8.234 &  8.638 &  8.792 &  8.245   \\ 
                               &  0.100 &  0.871 &  0.938 &  0.986 &  0.994 &  8.356 &  8.689 &  8.782 &  8.236   \\ 
\bottomrule 
\multirow{ 4}{*}{\( \nu=12\)}   &  0.010 &  0.588 &  0.797 &  0.916 &  0.964 &  5.914 &  7.437 &  8.173 &  8.342   \\ 
                                &  0.025 &  0.806 &  0.903 &  0.950 &  0.980 &  7.801 &  8.559 &  8.740 &  8.444   \\ 
                                &  0.050 &  0.863 &  0.919 &  0.972 &  0.985 &  8.334 &  8.684 &  8.766 &  7.997   \\ 
                                &  0.100 &  0.898 &  0.951 &  0.978 &  0.981 &  8.615 &  8.740 &  8.675 &  7.670   \\ 
\bottomrule 
\end{tabularx}
\raggedright
\scriptsize{ \textit{Notes:} This table displays the finite sample properties of the MCS for VaR forecasts evaluated using the GPL loss with \(b=0.5\) and the second set of models (crossref?). The level of the test is \( \alpha \)=0.25, the number of simulations is 1,000. Potency is the frequency at which \( \mathcal{M}^{*} \subset \widehat{\mathcal{M}}^{*}_{1-\alpha} \), power is defined as the average of \(|\widehat{\mathcal{M}}^{*}_{1-\alpha}|\).}
\end{table}


==> content/tables/simulation_true_model_10/summary_statistics/0/0/panel_mcs_90.tex <==
\begin{table}[h!]
\scriptsize
\centering
\caption{Simulation results for the second set of models: VaR evaluated using the GPL loss with \(b=0.5\).}
\label{tab:second}
\begin{tabularx}{1\textwidth}{l X X X X X X X X X }
\toprule 
        &  & \multicolumn{4}{c}{Potency} & \multicolumn{4}{c}{Power}   \\ 
                               &\(p \backslash P \) & 63 & 126 & 251 & 500 & 63 & 126 & 251 & 500   \\ 
\toprule 
\multirow{ 4}{*}{\( \nu=3\)}   &  0.010 &  0.632 &  0.837 &  0.942 &  0.971 &  6.987 &  8.623 &  9.343 &  9.448   \\ 
                               &  0.025 &  0.898 &  0.964 &  0.988 &  0.996 &  8.096 &  9.005 &  9.243 &  9.135   \\ 
                               &  0.050 &  0.954 &  0.987 &  0.996 &  1.000 &  8.330 &  8.861 &  8.859 &  8.700   \\ 
                               &  0.100 &  0.972 &  0.983 &  0.996 &  1.000 &  8.264 &  8.401 &  8.178 &  7.579   \\ 
\bottomrule 
\multirow{ 4}{*}{\( \nu=7\)}   &  0.010 &  0.653 &  0.842 &  0.938 &  0.978 &  6.771 &  8.309 &  9.131 &  9.252   \\ 
                               &  0.025 &  0.854 &  0.938 &  0.977 &  0.992 &  8.327 &  9.075 &  9.343 &  9.230   \\ 
                               &  0.050 &  0.904 &  0.959 &  0.991 &  0.999 &  8.776 &  9.180 &  9.344 &  9.093   \\ 
                               &  0.100 &  0.930 &  0.969 &  0.995 &  1.000 &  8.983 &  9.221 &  9.342 &  9.000   \\ 
\bottomrule 
\multirow{ 4}{*}{\( \nu=12\)}   &  0.010 &  0.677 &  0.857 &  0.947 &  0.990 &  6.502 &  8.010 &  8.798 &  9.028   \\ 
                                &  0.025 &  0.865 &  0.949 &  0.977 &  0.991 &  8.282 &  9.158 &  9.352 &  9.207   \\ 
                                &  0.050 &  0.921 &  0.963 &  0.990 &  0.996 &  8.929 &  9.274 &  9.354 &  9.053   \\ 
                                &  0.100 &  0.943 &  0.983 &  0.994 &  0.998 &  9.163 &  9.352 &  9.322 &  8.757   \\ 
\bottomrule 
\end{tabularx}
\raggedright
\scriptsize{ \textit{Notes:} This table displays the finite sample properties of the MCS for VaR forecasts evaluated using the GPL loss with \(b=0.5\) and the second set of models (crossref?). The level of the test is \( \alpha \)=0.1, the number of simulations is 1,000. Potency is the frequency at which \( \mathcal{M}^{*} \subset \widehat{\mathcal{M}}^{*}_{1-\alpha} \), power is defined as the average of \(|\widehat{\mathcal{M}}^{*}_{1-\alpha}|\).}
\end{table}


==> content/tables/simulation_true_model_10/summary_statistics/0/0/panel_mcs_95.tex <==
\begin{table}[h!]
\scriptsize
\centering
\caption{Simulation results for the second set of models: VaR evaluated using the GPL loss with \(b=0.5\).}
\label{tab:second}
\begin{tabularx}{1\textwidth}{l X X X X X X X X X }
\toprule 
        &  & \multicolumn{4}{c}{Potency} & \multicolumn{4}{c}{Power}   \\ 
                               &\(p \backslash P \) & 63 & 126 & 251 & 500 & 63 & 126 & 251 & 500   \\ 
\toprule 
\multirow{ 4}{*}{\( \nu=3\)}   &  0.010 &  0.663 &  0.854 &  0.952 &  0.980 &  7.183 &  8.777 &  9.435 &  9.602   \\ 
                               &  0.025 &  0.912 &  0.977 &  0.991 &  0.996 &  8.261 &  9.202 &  9.422 &  9.337   \\ 
                               &  0.050 &  0.970 &  0.992 &  0.998 &  1.000 &  8.692 &  9.076 &  9.090 &  8.935   \\ 
                               &  0.100 &  0.982 &  0.993 &  0.998 &  1.000 &  8.590 &  8.759 &  8.562 &  8.048   \\ 
\bottomrule 
\multirow{ 4}{*}{\( \nu=7\)}   &  0.010 &  0.694 &  0.865 &  0.953 &  0.987 &  7.053 &  8.492 &  9.305 &  9.450   \\ 
                               &  0.025 &  0.880 &  0.958 &  0.984 &  0.997 &  8.551 &  9.282 &  9.516 &  9.456   \\ 
                               &  0.050 &  0.936 &  0.971 &  0.994 &  1.000 &  9.058 &  9.399 &  9.537 &  9.372   \\ 
                               &  0.100 &  0.958 &  0.984 &  0.998 &  1.000 &  9.282 &  9.423 &  9.524 &  9.288   \\ 
\bottomrule 
\multirow{ 4}{*}{\( \nu=12\)}   &  0.010 &  0.735 &  0.892 &  0.963 &  0.995 &  6.807 &  8.258 &  9.064 &  9.295   \\ 
                                &  0.025 &  0.885 &  0.962 &  0.985 &  0.993 &  8.503 &  9.320 &  9.530 &  9.418   \\ 
                                &  0.050 &  0.947 &  0.976 &  0.998 &  1.000 &  9.201 &  9.465 &  9.571 &  9.343   \\ 
                                &  0.100 &  0.966 &  0.989 &  0.999 &  1.000 &  9.391 &  9.533 &  9.535 &  9.186   \\ 
\bottomrule 
\end{tabularx}
\raggedright
\scriptsize{ \textit{Notes:} This table displays the finite sample properties of the MCS for VaR forecasts evaluated using the GPL loss with \(b=0.5\) and the second set of models (crossref?). The level of the test is \( \alpha \)=0.05, the number of simulations is 1,000. Potency is the frequency at which \( \mathcal{M}^{*} \subset \widehat{\mathcal{M}}^{*}_{1-\alpha} \), power is defined as the average of \(|\widehat{\mathcal{M}}^{*}_{1-\alpha}|\).}
\end{table}


==> content/tables/simulation_true_model_10/summary_statistics/0/2/panel_mcs_75.tex <==
\begin{table}[h!]
\scriptsize
\centering
\caption{Simulation results for the second set of models: VaR evaluated using the GPL loss with \(b=2\).}
\label{tab:second}
\begin{tabularx}{1\textwidth}{l X X X X X X X X X }
\toprule 
        &  & \multicolumn{4}{c}{Potency} & \multicolumn{4}{c}{Power}   \\ 
                               &\(p \backslash P \) & 63 & 126 & 251 & 500 & 63 & 126 & 251 & 500   \\ 
\toprule 
\multirow{ 4}{*}{\( \nu=3\)}   &  0.010 &  0.546 &  0.743 &  0.861 &  0.901 &  6.275 &  7.936 &  8.687 &  8.787   \\ 
                               &  0.025 &  0.844 &  0.912 &  0.957 &  0.978 &  7.339 &  8.097 &  8.451 &  8.412   \\ 
                               &  0.050 &  0.895 &  0.962 &  0.982 &  0.991 &  7.371 &  7.775 &  7.869 &  7.709   \\ 
                               &  0.100 &  0.925 &  0.951 &  0.979 &  0.991 &  7.119 &  7.115 &  6.890 &  6.337   \\ 
\bottomrule 
\multirow{ 4}{*}{\( \nu=7\)}   &  0.010 &  0.557 &  0.753 &  0.855 &  0.937 &  6.131 &  7.585 &  8.304 &  8.496   \\ 
                               &  0.025 &  0.752 &  0.861 &  0.928 &  0.953 &  7.568 &  8.358 &  8.742 &  8.472   \\ 
                               &  0.050 &  0.818 &  0.890 &  0.948 &  0.972 &  8.012 &  8.498 &  8.764 &  8.576   \\ 
                               &  0.100 &  0.847 &  0.918 &  0.967 &  0.993 &  8.164 &  8.554 &  8.769 &  8.663   \\ 
\bottomrule 
\multirow{ 4}{*}{\( \nu=12\)}   &  0.010 &  0.577 &  0.791 &  0.889 &  0.952 &  5.823 &  7.342 &  7.943 &  8.117   \\ 
                                &  0.025 &  0.778 &  0.876 &  0.930 &  0.958 &  7.607 &  8.449 &  8.664 &  8.501   \\ 
                                &  0.050 &  0.834 &  0.892 &  0.952 &  0.981 &  8.172 &  8.565 &  8.848 &  8.523   \\ 
                                &  0.100 &  0.869 &  0.921 &  0.969 &  0.982 &  8.483 &  8.750 &  8.850 &  8.445   \\ 
\bottomrule 
\end{tabularx}
\raggedright
\scriptsize{ \textit{Notes:} This table displays the finite sample properties of the MCS for VaR forecasts evaluated using the GPL loss with \(b=2\) and the second set of models (crossref?). The level of the test is \( \alpha \)=0.25, the number of simulations is 1,000. Potency is the frequency at which \( \mathcal{M}^{*} \subset \widehat{\mathcal{M}}^{*}_{1-\alpha} \), power is defined as the average of \(|\widehat{\mathcal{M}}^{*}_{1-\alpha}|\).}
\end{table}


==> content/tables/simulation_true_model_10/summary_statistics/0/2/panel_mcs_90.tex <==
\begin{table}[h!]
\scriptsize
\centering
\caption{Simulation results for the second set of models: VaR evaluated using the GPL loss with \(b=2\).}
\label{tab:second}
\begin{tabularx}{1\textwidth}{l X X X X X X X X X }
\toprule 
        &  & \multicolumn{4}{c}{Potency} & \multicolumn{4}{c}{Power}   \\ 
                               &\(p \backslash P \) & 63 & 126 & 251 & 500 & 63 & 126 & 251 & 500   \\ 
\toprule 
\multirow{ 4}{*}{\( \nu=3\)}   &  0.010 &  0.610 &  0.807 &  0.918 &  0.949 &  6.836 &  8.408 &  9.183 &  9.317   \\ 
                               &  0.025 &  0.890 &  0.958 &  0.984 &  0.992 &  7.933 &  8.745 &  9.031 &  9.030   \\ 
                               &  0.050 &  0.945 &  0.981 &  0.994 &  1.000 &  8.093 &  8.525 &  8.623 &  8.479   \\ 
                               &  0.100 &  0.972 &  0.985 &  0.997 &  0.998 &  8.038 &  8.137 &  7.918 &  7.504   \\ 
\bottomrule 
\multirow{ 4}{*}{\( \nu=7\)}   &  0.010 &  0.647 &  0.835 &  0.928 &  0.973 &  6.735 &  8.229 &  9.010 &  9.200   \\ 
                               &  0.025 &  0.844 &  0.930 &  0.965 &  0.988 &  8.239 &  8.973 &  9.277 &  9.268   \\ 
                               &  0.050 &  0.885 &  0.941 &  0.979 &  0.992 &  8.676 &  9.053 &  9.289 &  9.225   \\ 
                               &  0.100 &  0.916 &  0.966 &  0.989 &  1.000 &  8.891 &  9.184 &  9.321 &  9.205   \\ 
\bottomrule 
\multirow{ 4}{*}{\( \nu=12\)}   &  0.010 &  0.695 &  0.869 &  0.942 &  0.977 &  6.490 &  7.974 &  8.687 &  8.935   \\ 
                                &  0.025 &  0.848 &  0.937 &  0.962 &  0.989 &  8.138 &  9.033 &  9.245 &  9.206   \\ 
                                &  0.050 &  0.898 &  0.944 &  0.987 &  0.993 &  8.828 &  9.201 &  9.377 &  9.232   \\ 
                                &  0.100 &  0.933 &  0.968 &  0.992 &  0.994 &  9.114 &  9.305 &  9.398 &  9.154   \\ 
\bottomrule 
\end{tabularx}
\raggedright
\scriptsize{ \textit{Notes:} This table displays the finite sample properties of the MCS for VaR forecasts evaluated using the GPL loss with \(b=2\) and the second set of models (crossref?). The level of the test is \( \alpha \)=0.1, the number of simulations is 1,000. Potency is the frequency at which \( \mathcal{M}^{*} \subset \widehat{\mathcal{M}}^{*}_{1-\alpha} \), power is defined as the average of \(|\widehat{\mathcal{M}}^{*}_{1-\alpha}|\).}
\end{table}


==> content/tables/simulation_true_model_10/summary_statistics/0/2/panel_mcs_95.tex <==
\begin{table}[h!]
\scriptsize
\centering
\caption{Simulation results for the second set of models: VaR evaluated using the GPL loss with \(b=2\).}
\label{tab:second}
\begin{tabularx}{1\textwidth}{l X X X X X X X X X }
\toprule 
        &  & \multicolumn{4}{c}{Potency} & \multicolumn{4}{c}{Power}   \\ 
                               &\(p \backslash P \) & 63 & 126 & 251 & 500 & 63 & 126 & 251 & 500   \\ 
\toprule 
\multirow{ 4}{*}{\( \nu=3\)}   &  0.010 &  0.661 &  0.835 &  0.938 &  0.967 &  7.142 &  8.620 &  9.306 &  9.476   \\ 
                               &  0.025 &  0.908 &  0.976 &  0.989 &  0.996 &  8.189 &  9.014 &  9.236 &  9.257   \\ 
                               &  0.050 &  0.962 &  0.985 &  0.998 &  1.000 &  8.478 &  8.818 &  8.899 &  8.791   \\ 
                               &  0.100 &  0.978 &  0.993 &  1.000 &  0.998 &  8.440 &  8.559 &  8.411 &  8.027   \\ 
\bottomrule 
\multirow{ 4}{*}{\( \nu=7\)}   &  0.010 &  0.705 &  0.871 &  0.945 &  0.982 &  7.052 &  8.485 &  9.222 &  9.430   \\ 
                               &  0.025 &  0.885 &  0.953 &  0.979 &  0.995 &  8.510 &  9.207 &  9.449 &  9.474   \\ 
                               &  0.050 &  0.922 &  0.961 &  0.993 &  0.996 &  8.964 &  9.288 &  9.482 &  9.389   \\ 
                               &  0.100 &  0.944 &  0.975 &  0.995 &  1.000 &  9.158 &  9.355 &  9.491 &  9.396   \\ 
\bottomrule 
\multirow{ 4}{*}{\( \nu=12\)}   &  0.010 &  0.753 &  0.906 &  0.961 &  0.988 &  6.840 &  8.285 &  8.952 &  9.245   \\ 
                                &  0.025 &  0.879 &  0.959 &  0.972 &  0.993 &  8.409 &  9.267 &  9.440 &  9.439   \\ 
                                &  0.050 &  0.927 &  0.966 &  0.994 &  0.997 &  9.085 &  9.382 &  9.532 &  9.434   \\ 
                                &  0.100 &  0.953 &  0.983 &  0.994 &  0.998 &  9.337 &  9.495 &  9.574 &  9.383   \\ 
\bottomrule 
\end{tabularx}
\raggedright
\scriptsize{ \textit{Notes:} This table displays the finite sample properties of the MCS for VaR forecasts evaluated using the GPL loss with \(b=2\) and the second set of models (crossref?). The level of the test is \( \alpha \)=0.05, the number of simulations is 1,000. Potency is the frequency at which \( \mathcal{M}^{*} \subset \widehat{\mathcal{M}}^{*}_{1-\alpha} \), power is defined as the average of \(|\widehat{\mathcal{M}}^{*}_{1-\alpha}|\).}
\end{table}


==> content/tables/simulation_true_model_10/summary_statistics/1/0/panel_mcs_75.tex <==
\begin{table}[h!]
\scriptsize
\centering
\caption{Simulation results for the set of \(m=10\) models: Var and ES forecasts evaluated using the AL score.}
\label{tab:first}
\begin{tabularx}{1\textwidth}{l X X X X X X X X X X X X X }
\toprule 
        &  & \multicolumn{6}{c}{Potency} & \multicolumn{6}{c}{Power}   \\ 
                               &\(p \backslash P \) & 63 & 126 & 251 & 500 & 1000 & 2500 & 63 & 126 & 251 & 500 & 1000 & 2500   \\ 
\toprule 
\multirow{ 4}{*}{\( \nu=3\)}   &  0.010 &  0.548 &  0.736 &  0.871 &  0.946 &  0.989 &  0.999 &  6.394 &  7.986 &  8.812 &  9.099 &  8.782 &  6.618   \\ 
                               &  0.025 &  0.755 &  0.869 &  0.936 &  0.983 &  0.996 &  0.998 &  7.632 &  8.522 &  8.938 &  8.989 &  8.362 &  5.725   \\ 
                               &  0.050 &  0.884 &  0.939 &  0.974 &  0.995 &  0.999 &  0.999 &  7.888 &  8.589 &  8.794 &  8.668 &  8.016 &  5.822   \\ 
                               &  0.100 &  0.920 &  0.967 &  0.986 &  0.997 &  0.999 &  0.995 &  7.850 &  8.287 &  8.288 &  8.022 &  7.286 &  4.212   \\ 
\bottomrule 
\multirow{ 4}{*}{\( \nu=7\)}   &  0.010 &  0.520 &  0.743 &  0.863 &  0.940 &  0.984 &  0.998 &  5.820 &  7.338 &  8.208 &  8.596 &  8.516 &  7.865   \\ 
                               &  0.025 &  0.774 &  0.893 &  0.953 &  0.980 &  0.993 &  0.995 &  7.619 &  8.452 &  8.711 &  8.363 &  7.477 &  5.524   \\ 
                               &  0.050 &  0.900 &  0.946 &  0.979 &  0.989 &  0.994 &  0.998 &  8.412 &  8.806 &  8.826 &  8.138 &  6.690 &  4.335   \\ 
                               &  0.100 &  0.905 &  0.956 &  0.979 &  0.992 &  0.994 &  0.998 &  8.577 &  8.842 &  8.776 &  8.075 &  6.794 &  4.624   \\ 
\bottomrule 
\multirow{ 4}{*}{\( \nu=12\)}   &  0.010 &  0.570 &  0.761 &  0.891 &  0.958 &  0.976 &  0.989 &  5.668 &  7.003 &  7.705 &  7.934 &  7.611 &  6.591   \\ 
                                &  0.025 &  0.811 &  0.914 &  0.961 &  0.978 &  0.983 &  0.982 &  7.533 &  8.287 &  8.401 &  7.826 &  6.609 &  4.607   \\ 
                                &  0.050 &  0.897 &  0.945 &  0.976 &  0.982 &  0.978 &  0.990 &  8.428 &  8.780 &  8.625 &  7.723 &  6.016 &  3.734   \\ 
                                &  0.100 &  0.901 &  0.949 &  0.980 &  0.987 &  0.987 &  0.986 &  8.520 &  8.753 &  8.579 &  7.572 &  6.000 &  3.894   \\ 
\bottomrule 
\end{tabularx}
\raggedright
\scriptsize{ \textit{Notes:} This table displays the finite sample properties of the MCS for Var and ES forecasts evaluated using the AL score and the set of \(m=10\) models. The level of the test is \( \alpha \)=0.25, the number of simulations is 2,500. Potency is the frequency at which \( \mathcal{M}^{*} \subset \widehat{\mathcal{M}}^{*}_{1-\alpha} \), power is defined as the average of \(|\widehat{\mathcal{M}}^{*}_{1-\alpha}|\).}
\end{table}


==> content/tables/simulation_true_model_10/summary_statistics/1/1/panel_mcs_75.tex <==
\begin{table}[h!]
\scriptsize
\centering
\caption{Simulation results for the second set of models: ES evaluated using the NZ score.}
\label{tab:second}
\begin{tabularx}{1\textwidth}{l X X X X X X X X X }
\toprule 
        &  & \multicolumn{4}{c}{Potency} & \multicolumn{4}{c}{Power}   \\ 
                               &\(p \backslash P \) & 63 & 126 & 251 & 500 & 63 & 126 & 251 & 500   \\ 
\toprule 
\multirow{ 4}{*}{\( \nu=3\)}   &  0.010 &  0.563 &  0.748 &  0.892 &  0.935 &  6.478 &  8.100 &  8.925 &  9.049   \\ 
                               &  0.025 &  0.818 &  0.897 &  0.961 &  0.979 &  7.692 &  8.502 &  8.882 &  8.707   \\ 
                               &  0.050 &  0.904 &  0.964 &  0.986 &  0.990 &  7.773 &  8.480 &  8.528 &  8.342   \\ 
                               &  0.100 &  0.922 &  0.958 &  0.987 &  0.996 &  7.663 &  7.975 &  7.803 &  7.237   \\ 
\bottomrule 
\multirow{ 4}{*}{\( \nu=7\)}   &  0.010 &  0.563 &  0.752 &  0.884 &  0.958 &  6.170 &  7.583 &  8.418 &  8.610   \\ 
                               &  0.025 &  0.785 &  0.895 &  0.956 &  0.980 &  7.801 &  8.498 &  8.799 &  8.468   \\ 
                               &  0.050 &  0.860 &  0.926 &  0.974 &  0.986 &  8.252 &  8.675 &  8.741 &  8.167   \\ 
                               &  0.100 &  0.879 &  0.944 &  0.986 &  0.994 &  8.360 &  8.718 &  8.775 &  8.201   \\ 
\bottomrule 
\multirow{ 4}{*}{\( \nu=12\)}   &  0.010 &  0.579 &  0.793 &  0.901 &  0.962 &  5.848 &  7.230 &  7.851 &  8.022   \\ 
                                &  0.025 &  0.828 &  0.924 &  0.965 &  0.982 &  7.793 &  8.535 &  8.693 &  8.204   \\ 
                                &  0.050 &  0.883 &  0.931 &  0.974 &  0.992 &  8.415 &  8.724 &  8.732 &  7.872   \\ 
                                &  0.100 &  0.906 &  0.958 &  0.979 &  0.986 &  8.629 &  8.801 &  8.689 &  7.680   \\ 
\bottomrule 
\end{tabularx}
\raggedright
\scriptsize{ \textit{Notes:} This table displays the finite sample properties of the MCS for ES forecasts evaluated using the NZ score and the second set of models (crossref?). The level of the test is \( \alpha \)=0.25, the number of simulations is 1,000. Potency is the frequency at which \( \mathcal{M}^{*} \subset \widehat{\mathcal{M}}^{*}_{1-\alpha} \), power is defined as the average of \(|\widehat{\mathcal{M}}^{*}_{1-\alpha}|\).}
\end{table}


==> content/tables/simulation_true_model_10/summary_statistics/1/1/panel_mcs_90.tex <==
\begin{table}[h!]
\scriptsize
\centering
\caption{Simulation results for the second set of models: ES evaluated using the NZ score.}
\label{tab:second}
\begin{tabularx}{1\textwidth}{l X X X X X X X X X }
\toprule 
        &  & \multicolumn{4}{c}{Potency} & \multicolumn{4}{c}{Power}   \\ 
                               &\(p \backslash P \) & 63 & 126 & 251 & 500 & 63 & 126 & 251 & 500   \\ 
\toprule 
\multirow{ 4}{*}{\( \nu=3\)}   &  0.010 &  0.591 &  0.795 &  0.925 &  0.960 &  6.830 &  8.488 &  9.274 &  9.465   \\ 
                               &  0.025 &  0.858 &  0.942 &  0.982 &  0.992 &  8.105 &  8.997 &  9.332 &  9.277   \\ 
                               &  0.050 &  0.940 &  0.982 &  0.992 &  0.998 &  8.390 &  8.941 &  9.041 &  8.906   \\ 
                               &  0.100 &  0.963 &  0.984 &  0.997 &  1.000 &  8.387 &  8.618 &  8.516 &  8.115   \\ 
\bottomrule 
\multirow{ 4}{*}{\( \nu=7\)}   &  0.010 &  0.636 &  0.819 &  0.921 &  0.976 &  6.644 &  8.104 &  8.931 &  9.147   \\ 
                               &  0.025 &  0.857 &  0.945 &  0.980 &  0.994 &  8.357 &  9.092 &  9.372 &  9.263   \\ 
                               &  0.050 &  0.917 &  0.969 &  0.992 &  0.999 &  8.840 &  9.240 &  9.376 &  9.107   \\ 
                               &  0.100 &  0.935 &  0.972 &  0.994 &  1.000 &  8.995 &  9.251 &  9.352 &  8.999   \\ 
\bottomrule 
\multirow{ 4}{*}{\( \nu=12\)}   &  0.010 &  0.665 &  0.843 &  0.939 &  0.986 &  6.351 &  7.803 &  8.547 &  8.770   \\ 
                                &  0.025 &  0.890 &  0.959 &  0.987 &  0.995 &  8.380 &  9.172 &  9.349 &  9.172   \\ 
                                &  0.050 &  0.940 &  0.972 &  0.994 &  0.997 &  9.008 &  9.310 &  9.355 &  9.011   \\ 
                                &  0.100 &  0.953 &  0.981 &  0.996 &  0.999 &  9.176 &  9.372 &  9.343 &  8.823   \\ 
\bottomrule 
\end{tabularx}
\raggedright
\scriptsize{ \textit{Notes:} This table displays the finite sample properties of the MCS for ES forecasts evaluated using the NZ score and the second set of models (crossref?). The level of the test is \( \alpha \)=0.1, the number of simulations is 1,000. Potency is the frequency at which \( \mathcal{M}^{*} \subset \widehat{\mathcal{M}}^{*}_{1-\alpha} \), power is defined as the average of \(|\widehat{\mathcal{M}}^{*}_{1-\alpha}|\).}
\end{table}


==> content/tables/simulation_true_model_10/summary_statistics/1/1/panel_mcs_95.tex <==
\begin{table}[h!]
\scriptsize
\centering
\caption{Simulation results for the second set of models: ES evaluated using the NZ score.}
\label{tab:second}
\begin{tabularx}{1\textwidth}{l X X X X X X X X X }
\toprule 
        &  & \multicolumn{4}{c}{Potency} & \multicolumn{4}{c}{Power}   \\ 
                               &\(p \backslash P \) & 63 & 126 & 251 & 500 & 63 & 126 & 251 & 500   \\ 
\toprule 
\multirow{ 4}{*}{\( \nu=3\)}   &  0.010 &  0.618 &  0.816 &  0.936 &  0.977 &  7.030 &  8.667 &  9.391 &  9.599   \\ 
                               &  0.025 &  0.885 &  0.954 &  0.990 &  0.995 &  8.304 &  9.141 &  9.462 &  9.449   \\ 
                               &  0.050 &  0.952 &  0.990 &  0.996 &  1.000 &  8.712 &  9.150 &  9.241 &  9.131   \\ 
                               &  0.100 &  0.972 &  0.991 &  0.998 &  1.000 &  8.642 &  8.906 &  8.857 &  8.546   \\ 
\bottomrule 
\multirow{ 4}{*}{\( \nu=7\)}   &  0.010 &  0.674 &  0.851 &  0.943 &  0.981 &  6.893 &  8.317 &  9.124 &  9.332   \\ 
                               &  0.025 &  0.890 &  0.957 &  0.987 &  0.997 &  8.582 &  9.317 &  9.532 &  9.466   \\ 
                               &  0.050 &  0.948 &  0.979 &  0.995 &  1.000 &  9.083 &  9.424 &  9.538 &  9.370   \\ 
                               &  0.100 &  0.963 &  0.984 &  0.996 &  1.000 &  9.284 &  9.432 &  9.533 &  9.296   \\ 
\bottomrule 
\multirow{ 4}{*}{\( \nu=12\)}   &  0.010 &  0.713 &  0.873 &  0.956 &  0.991 &  6.652 &  8.063 &  8.812 &  9.070   \\ 
                                &  0.025 &  0.909 &  0.970 &  0.992 &  0.997 &  8.626 &  9.350 &  9.543 &  9.390   \\ 
                                &  0.050 &  0.956 &  0.982 &  0.998 &  0.999 &  9.225 &  9.495 &  9.561 &  9.325   \\ 
                                &  0.100 &  0.968 &  0.990 &  0.997 &  1.000 &  9.410 &  9.550 &  9.555 &  9.228   \\ 
\bottomrule 
\end{tabularx}
\raggedright
\scriptsize{ \textit{Notes:} This table displays the finite sample properties of the MCS for ES forecasts evaluated using the NZ score and the second set of models (crossref?). The level of the test is \( \alpha \)=0.05, the number of simulations is 1,000. Potency is the frequency at which \( \mathcal{M}^{*} \subset \widehat{\mathcal{M}}^{*}_{1-\alpha} \), power is defined as the average of \(|\widehat{\mathcal{M}}^{*}_{1-\alpha}|\).}
\end{table}


==> content/tables/simulation_true_model_10/summary_statistics/1/2/panel_mcs_90.tex <==
\begin{table}[h!]
\scriptsize
\centering
\caption{Simulation results for the second set of models: ES evaluated using the FZG score.}
\label{tab:second}
\begin{tabularx}{1\textwidth}{l X X X X X X X X X }
\toprule 
        &  & \multicolumn{4}{c}{Potency} & \multicolumn{4}{c}{Power}   \\ 
                               &\(p \backslash P \) & 63 & 126 & 251 & 500 & 63 & 126 & 251 & 500   \\ 
\toprule 
\multirow{ 4}{*}{\( \nu=3\)}   &  0.010 &  0.570 &  0.762 &  0.909 &  0.963 &  6.786 &  8.484 &  9.362 &  9.633   \\ 
                               &  0.025 &  0.777 &  0.882 &  0.956 &  0.980 &  8.090 &  8.988 &  9.426 &  9.502   \\ 
                               &  0.050 &  0.930 &  0.973 &  0.989 &  0.992 &  8.498 &  9.050 &  9.213 &  9.169   \\ 
                               &  0.100 &  0.955 &  0.982 &  0.998 &  1.000 &  8.360 &  8.656 &  8.646 &  8.357   \\ 
\bottomrule 
\multirow{ 4}{*}{\( \nu=7\)}   &  0.010 &  0.601 &  0.777 &  0.913 &  0.968 &  6.480 &  7.925 &  8.849 &  9.146   \\ 
                               &  0.025 &  0.841 &  0.938 &  0.981 &  0.996 &  8.177 &  8.976 &  9.290 &  9.248   \\ 
                               &  0.050 &  0.935 &  0.974 &  0.993 &  1.000 &  8.921 &  9.330 &  9.424 &  9.148   \\ 
                               &  0.100 &  0.946 &  0.973 &  0.994 &  1.000 &  9.025 &  9.266 &  9.358 &  8.990   \\ 
\bottomrule 
\multirow{ 4}{*}{\( \nu=12\)}   &  0.010 &  0.620 &  0.807 &  0.927 &  0.983 &  6.218 &  7.589 &  8.367 &  8.751   \\ 
                                &  0.025 &  0.893 &  0.954 &  0.990 &  0.995 &  8.123 &  8.851 &  9.109 &  8.938   \\ 
                                &  0.050 &  0.960 &  0.983 &  0.994 &  0.997 &  9.116 &  9.396 &  9.370 &  8.954   \\ 
                                &  0.100 &  0.958 &  0.982 &  0.993 &  0.999 &  9.217 &  9.374 &  9.337 &  8.778   \\ 
\bottomrule 
\end{tabularx}
\raggedright
\scriptsize{ \textit{Notes:} This table displays the finite sample properties of the MCS for ES forecasts evaluated using the FZG score and the second set of models (crossref?). The level of the test is \( \alpha \)=0.1, the number of simulations is 1,000. Potency is the frequency at which \( \mathcal{M}^{*} \subset \widehat{\mathcal{M}}^{*}_{1-\alpha} \), power is defined as the average of \(|\widehat{\mathcal{M}}^{*}_{1-\alpha}|\).}
\end{table}


==> content/tables/simulation_true_model_10/summary_statistics/1/2/panel_mcs_95.tex <==
\begin{table}[h!]
\scriptsize
\centering
\caption{Simulation results for the second set of models: ES evaluated using the FZG score.}
\label{tab:second}
\begin{tabularx}{1\textwidth}{l X X X X X X X X X }
\toprule 
        &  & \multicolumn{4}{c}{Potency} & \multicolumn{4}{c}{Power}   \\ 
                               &\(p \backslash P \) & 63 & 126 & 251 & 500 & 63 & 126 & 251 & 500   \\ 
\toprule 
\multirow{ 4}{*}{\( \nu=3\)}   &  0.010 &  0.593 &  0.782 &  0.919 &  0.973 &  6.951 &  8.653 &  9.443 &  9.738   \\ 
                               &  0.025 &  0.802 &  0.905 &  0.970 &  0.985 &  8.298 &  9.153 &  9.526 &  9.616   \\ 
                               &  0.050 &  0.942 &  0.980 &  0.995 &  0.998 &  8.718 &  9.217 &  9.374 &  9.333   \\ 
                               &  0.100 &  0.968 &  0.989 &  0.998 &  1.000 &  8.651 &  8.931 &  8.934 &  8.663   \\ 
\bottomrule 
\multirow{ 4}{*}{\( \nu=7\)}   &  0.010 &  0.633 &  0.806 &  0.929 &  0.975 &  6.692 &  8.124 &  9.038 &  9.306   \\ 
                               &  0.025 &  0.878 &  0.959 &  0.987 &  0.999 &  8.443 &  9.220 &  9.503 &  9.481   \\ 
                               &  0.050 &  0.949 &  0.983 &  0.995 &  1.000 &  9.121 &  9.481 &  9.589 &  9.428   \\ 
                               &  0.100 &  0.969 &  0.984 &  0.996 &  1.000 &  9.300 &  9.457 &  9.539 &  9.291   \\ 
\bottomrule 
\multirow{ 4}{*}{\( \nu=12\)}   &  0.010 &  0.663 &  0.840 &  0.946 &  0.990 &  6.440 &  7.831 &  8.610 &  9.019   \\ 
                                &  0.025 &  0.913 &  0.970 &  0.995 &  0.997 &  8.385 &  9.094 &  9.369 &  9.272   \\ 
                                &  0.050 &  0.972 &  0.989 &  0.998 &  0.998 &  9.287 &  9.545 &  9.582 &  9.331   \\ 
                                &  0.100 &  0.971 &  0.992 &  0.997 &  0.999 &  9.413 &  9.559 &  9.559 &  9.223   \\ 
\bottomrule 
\end{tabularx}
\raggedright
\scriptsize{ \textit{Notes:} This table displays the finite sample properties of the MCS for ES forecasts evaluated using the FZG score and the second set of models (crossref?). The level of the test is \( \alpha \)=0.05, the number of simulations is 1,000. Potency is the frequency at which \( \mathcal{M}^{*} \subset \widehat{\mathcal{M}}^{*}_{1-\alpha} \), power is defined as the average of \(|\widehat{\mathcal{M}}^{*}_{1-\alpha}|\).}
\end{table}

